Intergranular stress distributions in polycrystalline aggregates of irradiated stainless steel

In order to predict InterGranular Stress Corrosion Cracking (IGSCC) of post-irradiated austenitic stainless steel in Light Water Reactor (LWR) environment, reliable predictions of intergranular stresses are required. Finite elements simulations have been performed on realistic polycrystalline aggregate with a recently proposed physically-based crystal plasticity constitutive equations validated for neutron-irradiated austenitic stainless steel. Intergranular normal stress probability density functions are found with respect to plastic strain and irradiation level, for uniaxial loading conditions. In addition, plastic slip activity jumps at grain boundaries are also presented. Intergranular normal stress distributions describe, from a statistical point of view, the potential increase of intergranular stress with respect to the macroscopic stress due to grain-grain interactions. The distributions are shown to be well described by a master curve once rescaled by the macroscopic stress, in the range of irradiation level and strain considered in this study. The upper tail of this master curve is shown to be insensitive to free surface effect, which is relevant for IGSCC

==> lamacro.tex <==
%DIAGRAMMES
\def\hfl#1#2{\smash{\mathop{\hbox to 12mm{\rightarrowfill}}
\limits^{\scriptstyle#1}_{\scriptstyle#2}}}
\def\vflb#1#2{\llap{$\scriptstyle #1$}\left\downarrow
\vbox to 6mm{}\right.\rlap{$\scriptstyle #2$}}
\def\vflh#1#2{\llap{$\scriptstyle #1$}\left\uparrow
\vbox to 6mm{}\right.\rlap{$\scriptstyle #2$}}
\def\diagram#1{\def\normalbaselines{\baselineskip=0pt
\lineskip=10pt\lineskiplimit=1pt}\matrix{#1}}
%FIN DIAGRAMMES
%
%FONTES
\tolerance=9999
\font\grostitre=cmbx10 scaled \magstep3
\font\titre=cmbx10 scaled \magstep2
\font\petittitre=cmbx10 scaled \magstep1
\font\petititre=cmbx10 scaled \magstep1
\font\twelverm=cmr10 scaled 1200
%FIN FONTES
%
%TAILLES ET BLANCS
\def\haut{\vphantom {\Bigl(}}
\def\bk{\bigskip}
%
%CHAPITRES-EQUATIONS
\newcount\chapno
\newcount\noeq
\def\gtitre{\hyphenpenalty=9999 \grostitre}

\def\eqincr{{\global\advance\noeq by 1} 
             \eqno{(\number\chapno.\number\noeq)}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
%FIN CHAPITRE-EQUATIONS
%
%FORMULES
\def\ten#1{\oalign{$\bf #1$\crcr\hidewidth$\scriptscriptstyle\sim$\hidewidth}\vphantom{#1}}
\def\tenormal#1{\oalign{$ #1$\crcr\hidewidth$\scriptscriptstyle\sim$\hidewidth}}
\def\tenb#1{\oalign{\mbox{\boldmath $ #1$}\crcr\hidewidth$\scriptscriptstyle\sim$\hidewidth}}
\def\tenu#1#2{{\ten#1}_{{\null}^{\scriptstyle #2}}}
\def\dtenu#1#2{{\dten#1}_{{\null}^{\scriptstyle #2}}}
\def\vectu#1#2{{\vect#1}_{{\null}^{\scriptstyle #2}}}
\def\dvecu#1#2{{\dvec#1}_{{\null}^{\scriptstyle #2}}}
%\def\ordta#1{\oalign{$\bf #1$\cr\hfill$\scriptscriptstyle\sim$\hfill\crcr\hfill$\bf \scriptscriptstyle -$\hfill}}
%\def\ordta#1{\oalign{$\bf #1$\cr\hfill$\scriptscriptstyle\sim$\hfill\crcr\hfill$\bf \scriptscriptstyle -$\hfill}}
\def\ordta#1{\oalign{$\bf #1$\crcr\hidewidth$\scriptscriptstyle{\underline \sim}$\hidewidth}}
\def\ordtab#1{\oalign{\mbox{\boldmath $ #1$}\crcr\hidewidth$\scriptscriptstyle{\underline \sim}$\hidewidth}}
\def\ordtb#1{\oalign{$\bf #1$\crcr\hidewidth$\scriptscriptstyle{\overline \sim}$\hidewidth}}
\def\ordtbb#1{\oalign{\mbox{\boldmath $ #1$}\crcr\hidewidth$\scriptscriptstyle{\overline \sim}$\hidewidth}}
%\def\ordtb#1{\oalign{$\bf #1$\cr\hfill$\scriptscriptstyle -$\hfill\cr\hfill$\bf \scriptscriptstyle\sim$\hfill}}
\def\dten#1{\oalign{$\bf{\dot{#1}}$\crcr\hidewidth$\scriptscriptstyle\sim$\hidewidth}\vphantom{#1}}
\def\dtenb#1{\oalign{\mbox{\boldmath ${\dot{#1}}$}\crcr\hidewidth$\scriptscriptstyle\sim$\hidewidth}}
\def\ordq#1{\ten{\ten #1}\vphantom{#1}}
\def\ordqu#1#2{{\ordq#1}_{{\null}^{\scriptstyle #2}}} % \ordqu{exp}{indice}
\def\dordqu#1#2{{\dordq#1}_{{\null}^{\scriptstyle #2}}}
%\def\ordq#1{\ten{\ten#1}\vphantom{#1}}
\def\vect#1{{\bf \underline #1}{\vphantom{#1}}}
\def\vectb#1{{\mbox{\boldmath  \underline {$ #1$}}}}
\def\dvect#1{{\bf \underline{\dot{#1}}}\vphantom{#1}}

\def\q{\quad}
\def\tr{{\rm Tr \,}}
\def\sup{\mathop{\hbox{\rm Sup}}\limits}
\def\symm#1{^\{{#1}^\}}
\def\asymm#1{^\}{#1}^\{}
\def\transp#1{{#1}^T}
\def\corot#1{{\,}^{c}#1}
\def\diese#1{{\ }^{\sharp}#1}
\def\etoil#1{{\ }^{\star}#1}
\def\vectasym#1{\mathop{#1}^{\times}}
\def\tild#1{{\mathop{#1}^{\sim}}}
\def\vcross#1{\buildrel\times\over{\underline{#1}}{}}
\def\rang{{\rm rang \,}}
\def\div{{\rm div}}
\def\grad{{\rm grad}}
\def\hess{{\rm hessian} }
\def\dt#1{\oalign{${\dot{#1}}$}}
\def\sym#1{{{}^\{#1{}^\}}}
\def\asym#1{{{}^\}#1{}^\{}}
\def\surplus#1{\mathop{#1}^{+}}
\def\nab{\vect \nabla}

% AUTRES MATHS (JB)
\def\VEC#1{ \left\{#1\right\} }
\def\MAT#1{ \left[#1\right] }
\def\Norm#1{\left|\left|#1\right|\right|}
\def\R{{\rm I \hspace{-.25em}R}}

%FIN FORMULES
%
%ABREVIATIONS
\def\eme{$^{\mbox{\small \`eme}}$}
\def\ere{$^{\mbox{\small \`ere}}$}
\def\er{$^{\mbox{\small er}}$}
%UNITES
\def\degreC{\hbox{${}^{\circ}$C\,}}
\def\degre{\hbox{${}^{\circ}$}}
\def\micron{\hbox{$\, \mu {\rm m}$}}
\def\metre{\hbox{$\, {\rm m}$}}
\def\metr{\hbox{$\, {\rm m}$}}
%FIN UNITES
%
%TABLEAUX
\def\tvi{\vrule height 12pt depth 5pt width 0pt}
\def\tv{\tvi\vrule}
\def\cc#1{\hfill\quad#1\quad\hfill}
%
%DEFORMATIONS ET LEURS VITESSES
\def\epsp{\dot{\varepsilon}}
\def\eplp{\dot{\varepsilon}^p}
\def\evip{\dot{\varepsilon}^v}
%MOTS LONGS COURANTS
\def\mhe {homogeneous equivalent medium }
\def\mhel {homogeneous equivalent medium}
\def\sc {self-consistent }
\def\gsc {generalized self-consistent }
\def\gscl {generalized self-consistent}
\def\ctd {continuum theory of dislocations }
\def\ctdl {continuum theory of dislocations}
%FIN TABLEAUX
\def\insec{~}
\def\Diamond{\diamond}
\def\Box{\oplus}
\def\SetFigFont#1#2#3{\null}
%
\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}
%NOTATIONS PROPRES ZEBULON
\def\vint{{\cal V}_{\rm int}}
\def\vaux{{\cal V}_{\rm aux}}
\def\ep{{\tt EP}}
\def\coef{{\tt CO}}
\def\prim{{\tt primal}}
\def\dual{{\tt dual}}
%
% Macros JLC
%
\def\cdm { M\'ecanique de l'Endommagement \,}
\def\fty { force thermodynamique associ\'ee \`a l'endommagement \,}
\def\ordqdot#1{\dot{\ten{\ten#1}}}
\def\ordqtilde#1{\tilde{\ten{\ten#1}}}
\def\tsigma{\smash{\ten{\sigma}}}
\def\tepsi{\smash{\ten{\varepsilon}}}
\def\groblan{\; \; \; \; \; \; \; \; }
\def\oqlambdai{\smash{{\ordq{\Lambda}}^{i}}}
\def\oqlambda{\smash{\ordq{\Lambda}}}


